The gradient flow coupling in the Schr\"odinger Functional

We study the perturbative behavior of the Yang-Mills gradient flow in the Schr\"odinger Functional, both in the continuum and on the lattice. The energy density of the flow field is used to define a running coupling at a scale given by the size of the finite volume box. From our perturbative computation we estimate the size of cutoff effects of this coupling to leading order in perturbation theory. On a set of Nf=2 gauge field ensembles in a physical volume of L ~ 0.4 fm we finally demonstrate the suitability of the coupling for a precise continuum limit due to modest cutoff effects and high statistical precision.

==> definition.tex <==

The Schrodinger Functional~\cite{aa} can be seen as the kernel of the
propagation 

In the Schrodinger functional the gauge field $A_\mu(x)$ is periodic
in the three spatial directions and has either Dirichlet or Neumann
boundary conditions in the time direction. These special boundary
conditions have to be preserved by the Wilson flow. 






% Local Variables: 
% mode: latex
% TeX-master: "paper"
% End: 


 

==> lb.tex <==




\begin{table}
  \centering
  \input{tab-lb.tex}
  \caption{Parameters of the fits to the large $\beta$ simulations.}
  \label{tab:lb}
\end{table}


% Local Variables: 
% mode: latex
% TeX-master: "paper"
% End: 


 
